Unsupervised Learning for Robust Fitting:A Reinforcement Learning Approach

Robust model fitting is a core algorithm in a large number of computer vision applications. Solving this problem efficiently for datasets highly contaminated with outliers is, however, still challenging due to the underlying computational complexity. Recent literature has focused on learning-based algorithms. However, most approaches are supervised which require a large amount of labelled training data. In this paper, we introduce a novel unsupervised learning framework that learns to directly solve robust model fitting. Unlike other methods, our work is agnostic to the underlying input features, and can be easily generalized to a wide variety of LP-type problems with quasi-convex residuals. We empirically show that our method outperforms existing unsupervised learning approaches, and achieves competitive results compared to traditional methods on several important computer vision problems.

==> method.tex <==
\section{Consensus maximization tree search as a Markov Decision Process}
In this section, we formulate consensus maximization tree search algorithm as a Markov Decision Process (MDP), which is defined by a tuple (S, T, A, R), where S is the set of State, T is the transition function, A is the set of actions, and R is the reward function.

\subsection{Graph representation as a state} 
Let $s_{t} $ be the state at time t. Each state includes some properties: (1) the N measurements, (2) all the previous actions have been selected so far, (3) available actions can be selected in the next state. 
We encode all these information as a graph representation so that it can become the input of the agent.


==> tex/figures/tableReal.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|ll}
\cline{1-3}
\textbf{Method} & \textbf{Number of inliers} & \textbf{Runtime} &  &  \\ \cline{1-3}
Ours            & 4948                       & 1.81             &  &  \\ \cline{1-3}
ULCM            & 4475                       & 0.20             &  &  \\ \cline{1-3}
RANSAC          & 4863                       & 1.90             &  &  \\ \cline{1-3}
\end{tabular}
\end{table}
